Intersection Graphs of Rays and Grounded Segments

We consider several classes of intersection graphs of line segments in the plane and prove new equality and separation results between those classes. In particular, we show that: (1) intersection graphs of grounded segments and intersection graphs of downward rays form the same graph class, (2) not every intersection graph of rays is an intersection graph of downward rays, and (3) not every intersection graph of rays is an outer segment graph. The first result answers an open problem posed by Cabello and Jej\v{c}i\v{c}. The third result confirms a conjecture by Cabello. We thereby completely elucidate the remaining open questions on the containment relations between these classes of segment graphs. We further characterize the complexity of the recognition problems for the classes of outer segment, grounded segment, and ray intersection graphs. We prove that these recognition problems are complete for the existential theory of the reals. This holds even if a 1-string realization is given as additional input.

==> UnUsed.tex <==
\newpage
\section{Unused}
\till{Here comes, what we are not currently using, but maybe want to keep in mind for later.
Eventually it will get deleted.}




\begin{framed}


% \till{It seems I don't need the lemma after all.
% 
% I keep it for now, maybe it turns out to be useful later.}

  \includegraphics{Disjointness}
% \begin{figure}[htbp]
%   \centering
% 
%   \caption{Illustration of \Cref{lem:disjointness}. The edges $12$ and $ab$ are present but non of the other edges.}
%   \label{fig:disjointness}
% \end{figure}

\begin{lemma}[Disjointness]\label{lem:disjointness}
  Let $G$ be a graph and $1,2,a,b\in V(G)$ with $12,ab \in E(G)$ and $1a,1b,2a,2b \notin E(G)$. Further assume that $R$ is a representation of $G$ as outer-$1$-string graph or grounded-$1$-string graph.
  Then the base points must be in the order $12ab$, up to symmetry.
\end{lemma}
\begin{proof}
 The only order of the base points on $S^1$ or the $x$-axis is, up to symmetry, $1a2b$. For the purpose of contradiction, suppose there exists a representation of as grounded-$1$-string graphs. (The proof for outer-$1$-string graphs is analogous.) Then the outer segments $1$ and $2$ together with the grounding line contain a closed curve that separates the plane into two parts. The two $1$-outer segments $a$ and $b$ are in the two different components and thus cannot have a common point --- a contradiction.
\end{proof}
\end{framed}

\begin{framed}

% \till{This is the old summary from Jean}

Consider an $n$-cycle $C$, and a graph $ G = (V,E)$ on $n$ vertices that are $1$-to-$1$ adjacent with vertices of the cycle. Consider any outer pseudosegment representation of this graph. Then portions of the curves representing $C$ form a closed curve $D$, and the curves corresponding to vertices of $V$ are contained in the interior of $D$, and intersect $D$ in the order prescribed by the cycle.

outersegment graphs
grounded segment graphs

ray graphs
downward ray graphs

outer pseudosegment graphs
grounded pseudosegment graphs

discussion on pseudosegments:
- extendable pseudosegment vs 1-string
- strong/weak grounded extendable pseudosegments

---
Order-forcing cycle construction
---

This construction is used throughout.

Lemma
Consider an n-cycle C, and a graph on n vertices V that are 1-to-1 adjacent with vertices of the cycle. Consider any outer pseudosegment representation of this graph. Then portions of the curves representing C form a closed curve D, and the curves corresponding to vertices of V are contained in the interior of D, and intersect D in the order prescribed by the cycle.

The same holds for outersegment and grounded segment graphs.
\end{framed}


\begin{framed}
 
---
Stretchability issues
---

Statements
Outer pseudosegment graphs $\neq$ outersegment graphs.
Grounded pseudosegment graphs $\neq$ grounded segment graphs.

Proof: from an arbitrary pseudoline arrangement A, we can construct an outer pseudosegment graph that is stretchable iff A is. Use the order-forcing cycle, plus a pair of "probe" segments witnessing each successive crossing. Check that this can be stretched whenever A can be stretched. Check that this can be drawn both on a line and inside a circle.

Corollary
Recognition of outer/grounded pseudosegment graphs is ETR-complete. This holds even if we give a description of the realization with pseudosegments.

% \till{The corollary also holds for general rays.
% Also I think recognition of grounded segment graphs is hard. Not the pseudo variant. (The pseudo variant is in NP.)}
\end{framed}

\begin{framed}
1) downward ray graphs = grounded segment graphs

Proof: Assume all segments are grounded on the x-axis and lie above it. Use the projective transformation mapping (x, y) to (x/y, -1/y).

This answers Cabello and Jejcic's second question.

2) ray graphs $\neq$ outersegment graphs

Clearly, ray graphs are outersegment. But some outersegment graphs are not ray graphs.

Proof: Use the order-forcing cycle and construct a 4-tuple a,b,c,d of segments in a circle such that a crosses b, c crosses d, and the angles between a,b and c,d are both less than pi. This forces one pair of rays to intersect in any ray representation. See figure in Till's email.

3) downward ray graphs $\neq$ ray graphs

Proof: Use the order forcing cycle again, but implement it carefully so that it works for rays instead of segments in a circle. This uses Stefan's idea for controlling the slopes by considering a regular polygon. Then we can implement the 4-way crossing with arbitrary rays, but not downward rays (see again Till's picture).

Note: this was originally done for distinguishing outersegment from grounded segments, thereby answering Cabello and Jejcic's first question. But now we get this distinction by transitivity from the two others above.
\end{framed}
